Rally and WebScience: A Platform and Toolkit for Browser-Based Research on Technology and Society Problems

Empirical technology and society research is in a methodological crisis. Problems increasingly involve closed platforms, targeted content, and context-specific behavior. Prevailing research methods, such as surveys, tasks, and web crawls, pose design and ecological validity limitations. Deploying studies in participant browsers and devices is a promising direction. These vantage points can observe individualized experiences and implement UI interventions in real settings. We survey scholarship that uses these methods, annotating 284 sampled papers. Our analysis demonstrates their potential, but also recurring implementation barriers and shortcomings. We then present Rally and sdkName, a platform and toolkit for browser-based research. These systems lower implementation barriers and advance the science of measuring online behavior. Finally, we evaluate Rally and sdkName against our design goals. We report results from a one-month pilot study on news engagement, analyzing 4,466,200 webpage visits from 1,817 participants. We also present observations from interviews with researchers using these systems.

==> figures/arch.tex <==
\newcommand\csDesc{
    \begin{varwidth}{0.25\linewidth}
        \textbf{Content Scripts}
        \begin{itemize}
            \item registered to domain match patterns
            \item scrape content from page
            \item subscribe to page events
        \end{itemize}
    \end{varwidth}
}

\newcommand\csTobg{
    \begin{varwidth}{0.1\linewidth}\small
        Page contents, metadata
    \end{varwidth}
}

\newcommand\bgTocs{
    \begin{varwidth}{0.1\linewidth}\small
        Requests to perform tasks or send specific content
    \end{varwidth}
}

\newcommand\bgDesc{
    \begin{varwidth}{0.25\linewidth}
        \textbf{Background Pages}
        \begin{itemize}
            \item inject content scripts
            \item listen for content script messages
            \item subscribe to browser events
            \item perform initial processing
        \end{itemize}
    \end{varwidth}
}

\newcommand\wwTobg{
    \begin{varwidth}{0.1\linewidth}\small
        Results of processing
    \end{varwidth}
}
\newcommand\bgToww{
    \begin{varwidth}{0.1\linewidth}\small
        Data and requests to process
    \end{varwidth}
}

\newcommand\wwDesc{
    \begin{varwidth}{0.25\linewidth}
        \textbf{Web Workers}
        \begin{itemize}
            \item handle longer-running secondary processing tasks
        \end{itemize}
    \end{varwidth}
}

\newcommand\bgTobs{
    \begin{varwidth}{0.1\linewidth}\small
        Store raw records
    \end{varwidth}
}

\newcommand\bsDesc{
    \begin{varwidth}{0.25\linewidth}
        \textbf{Browser storage}
        \begin{itemize}
            \item raw records of measurements
            \item deleted once processed
        \end{itemize}
    \end{varwidth}
}

\newcommand\bsTotp{
    \begin{varwidth}{0.1\linewidth}\small
        Sends processed (aggregated) records
    \end{varwidth}
}

\newcommand\tpDesc{
    \begin{varwidth}{0.25\linewidth}
        \textbf{Telemetry Pings}
        \begin{itemize}
            \item aggregated records sent periodically
            \item encrypted in transit
        \end{itemize}
    \end{varwidth}
}

\newcommand\tpToae{
    \begin{varwidth}{0.1\linewidth}\small
        Sent via Telemetry
    \end{varwidth}
}

\newcommand\aeDesc{
    \begin{varwidth}{0.25\linewidth}
        \textbf{Analysis Environment}
        \begin{itemize}
            \item aggregated records from all users
            \item access-controlled
            \item analysis tools
            \item analysis results, not raw data, can leave
        \end{itemize}
    \end{varwidth}
}

\tikzset{storageNode/.style={shape=rectangle,
                             draw=red, semithick,
                             align=center}}

\tikzset{labelNode/.style={draw=none, fill=none}}
\begin{figure*}
\begin{tikzpicture}[
        every node/.style = {shape=rectangle,
                             draw=black, semithick,
                             align=center}
                         ]
    \node (cs) [draw] {\csDesc{}};
    \node (bg) [right=0.12\linewidth of cs] {\bgDesc{}};
    \node (ww) [right=0.12\linewidth of bg] {\wwDesc{}};
    \node (bs) [storageNode, below=2cm of cs] {\bsDesc{}};
    \node (tp) [storageNode, right=0.12\linewidth of bs] {\tpDesc{}};
    \node (ae) [storageNode, right=0.12\linewidth of tp] {\aeDesc{}};

    \draw[->] ([yshift=0.2cm]cs.east) -- ([yshift=0.2cm]bg.west) node [above, midway, labelNode] {\csTobg{}};
    \draw[->] ([yshift=-0.25cm]bg.west) -- ([yshift=-0.25cm]cs.east) node [midway, below, labelNode] {\bgTocs{}};

    \draw[->] ([yshift=0.2cm]bg.east) -- ([yshift=0.2cm]ww.west) node [above, midway, labelNode] {\bgToww{}};
    \draw[->] ([yshift=-0.25cm]ww.west) -- ([yshift=-0.25cm]bg.east) node [midway, below, labelNode] {\wwTobg{}};

    \draw[->] (bg.south) -- (bs.north) node [above, near end, labelNode] {\bgTobs{}};
    
    \draw[->] (bs.east) -- (tp.west) node [below, midway, labelNode] {\bsTotp{}};

    \draw[->] (tp.east) -- (ae.west) node [below, midway, labelNode] {\tpToae{}};
    
\end{tikzpicture}

\caption{The flow of data through \sdkName{}. Black boxes represent processing units;
red boxes represent data storage or transport units.
\note{AK: Deciding whether to keep this/similar diagram or scrap it, opinions welcome}
}
\label{fig:sdk_data_flow}
\end{figure*}


==> figures/browsing-table.tex <==

\begin{tabular}{r|l|l|l|l|} 
	\cline{2-5}
	\vcell{\textbf{\Large{WebScience}}}   & \vcell{\begin{tabular}[b]{@{}l@{}}pageId: 1\\url: www.a.com\\referrer: none\\priorPageId: none\\transitionType: typed\\transitionQualifier: from\_address\_bar\\startTime: 1/15/21 16:21:31\\\end{tabular}} & \vcell{\begin{tabular}[b]{@{}l@{}}pageId: 2\\url: www.b.com\\referrer: www.a.com\\priorPageId: 1\\transitionType: link\_click\\startTime: 1/15/21 16:22:01\\attentionDuration: 1700\\maxScrollDepth: 23\\\end{tabular}} & \vcell{\begin{tabular}[b]{@{}l@{}}pageId: 1\\url: www.a.com\\referrer: none\\priorPageId:2\\startTime: 1/15/21 16:21:31\\stopTime: 1/15/21 16:23:03\\attentionDuration: 7500\\maxScrollDepth: 76\\\end{tabular}} & \vcell{\begin{tabular}[b]{@{}l@{}}pageId: 3\\url: www.c.com\\referrer: www.a.com\\priorPageId: 1\\transitionType: link\_click\\startTime: 1/15/21 16:23:03\\stopTime: 1/15/21 16:27:03\\attentionDuration: 24000\\maxScrollDepth: 91\end{tabular}}  \\[-\rowheight]
	\printcelltop        & \printcelltop                                                                                                                                                                                                                                                 & \printcelltop                                                                                                                                                                                                               & \printcelltop                                                                                                                                                                                              & \printcelltop                                                                                                                                                                                                               \\ 
	\cline{2-5}
	\vcell{\textbf{\Large{Conventional}}} & \vcell{\begin{tabular}[b]{@{}l@{}}pageId: 1\\url: www.a.com\\time: 1/15/21 16:21:31\\referrer: none\\priorPageLoaded: none\\\end{tabular}}                                                                                                                                         & \vcell{\begin{tabular}[b]{@{}l@{}}pageId: 2\\url: www.b.com\\time: 1/15/21 16:22:01\\referrer: www.a.com\\priorPageLoaded: 1\\timeSincePriorPageLoad: 3000\\\end{tabular}}                                                                                                      & \vcell{--}                                                                                                                                                                                                 & \vcell{\begin{tabular}[b]{@{}l@{}}pageId: 3\\url: www.c.com\\time: 1/15/21 16:23:03\\referrer: www.a.com\\priorPageLoaded: 2\\timeSincePriorPageLoad: 62000\\\end{tabular}}                                                                                                                       \\[-\rowheight]
	\printcelltop        & \printcelltop                                                                                                                                                                                                                                                 & \printcelltop                                                                                                                                                                                                               & \printcellmiddle                                                                                                                                                                                           & \printcelltop                                                                                                                                                                                                               \\
	\cline{2-5}
\end{tabular}

==> figures/lifecycle.tex <==
  \begin{tikzpicture}[
      node distance=2.0in,
      thick]
    \tikzstyle{every node}=[base]
    \node (start)[]{};
    \node (enrollment-details) [xshift=-0.75in, below right of=start] {
      \makecell[c]{
        \textbf{Rally}\\
        Acquire participants\\
        Explain studies\\
        Gain consent
    }};
    \node (collection-ws-details) [right of=enrollment-details] {
      \makecell[c]{
        \textbf{\large WebScience}\\
        Measure participant activity\\
        Deploy interventions\\
        \hfill 
    }};
    \node (collection-st-details) [right of=collection-ws-details] {
      \makecell[c]{
        \textbf{\large Study Code}\\
        Configure WebScience modules\\
        Build custom measurements\\
        Create activity digests for reporting
    }};
    \node (reporting-details) [right of=collection-st-details] {
      \makecell[c]{
        \textbf{\large Rally}\\
        Report digests to backend\\
        Mediate access to study data\\
        \hfill 
    }};
    \node (end) [yshift=-0.9in, xshift=-1.35in, above right of=reporting-details] {};

    \draw[-] node[above of=collection-ws-details,yshift=-1.05in,xshift=1in] {\LARGE\emph{Stages of Study Implementation}};
    \draw[-] node[above of=enrollment-details,yshift=-1.30in] {\Large\textbf{Enrollment}};
    \draw[-] node[above of=collection-ws-details,yshift=-1.30in,xshift=1in] {\Large\textbf{Data Collection}};
    \draw[-] node[above of=reporting-details, yshift=-1.30in] {\Large\textbf{Reporting}};
    \draw[-] (enrollment-details) |- (end);
    \draw[-] (collection-ws-details) |- (end);
    \draw[-] (collection-st-details) |- (end);
    \draw[-] (reporting-details) |- (end);


  \end{tikzpicture}



==> figures/meas-methods/figure-attn-dt-ttnl-histo.tex <==

\begin{tikzpicture}
\begin{axis}
    [
    ybar interval,
    xtick={-160, -150, -140, -130, -120, -110, -100, -90, -80, -70, -60, -50, -40, -30, -20, -10, 0, 10, 20, 30, 40, 50, 60, 70, 80, 90, 100},
    ymax=2800000,
    xticklabels={< -150, -140, -130, -120, -110, -100, -90, -80, -70, -60, -50, -40, -30, -20, -10, 0, 10, 20, 30, 40, 50, 60, 70, 80, 90, >=100},
    x tick label style={rotate=90,},
    xlabel = {The upper bound of the error interval.},
    ylabel = {Number of visits in each error interval.},
    width=300pt,
    height=200pt,
    ] 
    \addplot [draw=black, fill=cb3] coordinates {
    (-160 124827)
    (-150, 3311) (-140, 3578) (-130, 3937) (-120, 4279) (-110, 4721) (-100, 5222) (-90, 5840) (-80, 6841) (-70, 7956) (-60, 9543) (-50, 11368) (-40, 13338) (-30, 16031) (-20, 21768) (-10, 36486) (0, 2520373) (10, 183037) (20, 89794) (30, 61196) (40, 50601) (50, 48317) (60, 53332) (70, 63487) (80, 90444) (90, 338441)
    (100, 194)
    };
\end{axis}
\end{tikzpicture}

==> figures/survey/survey-consent-table.tex <==
\footnotesize
	\newcolumntype{C}{>{\centering\arraybackslash}m{0.15\linewidth}}
	\begin{tabular}{l C C C C }
		&
		consent obtained &
		consent explained &
		consent not obtained &
		consent not stated
		\\ \hline
		% ./eqn.py -f coded-05-nomooc-ecom.csv -t "consent" -n "participants"
		% ./eqn.py -f coded-05-nomooc-ecom.csv -t "consent" -n "participants" --no-ext
		Count (\%) &
		  244 (32.5\%) &
		  41 (5.5\%) &
		  5 (0.7\%) &
		  461 (61.4\%)
		  \\ \hline
		Median participants (count) &
		  624 &
		  736 &
		  28100000 &
		  2654 
		  \\ \hline
		  % ./eqn.py -f coded-05-nomooc-ecom.csv -t "consent" -n "timespan"
		  % ./eqn.py -f coded-05-nomooc-ecom.csv -t "consent" -n "timespan" --no-ext
		Median duration (count) &
		  91 &
		  90 &
		  34 &
		  150 
		  \\ \hline
	\end{tabular}


==> figures/survey/table-data-source-discipline.tex <==

\footnotesize
% ./eqn.py -f coded-05.csv -t "data source" -c "discipline"
	\newcolumntype{C}{>{\centering\arraybackslash}m{0.1\linewidth}}
	\begin{tabular}{l C C C C C C}
	                    & Research data provider & Partnership & Custom instrumentation & Not stated & MOOC & E-commerce
		\\ \hline
		Applied science & 172 (13.5\%)           & 227 (17.8\%) & 210 (16.5\%)          & 23 (1.8\%) & 250 (19.6\%) & 196 (15.4\%)
		\\ \hline
		Social science  & 67 (5.3\%)             & 23 (1.8\%)   & 13 (1.0\%)            &            &              & 78 (6.1\%)
		\\ \hline
		Math            & 10 (0.8\%)             &              &                       &            &  &
		\\ \hline
		Humanities      & 1 (0.1\%)              &              &                       &            &  &
		\\ \hline
		Natural science &                        & 1 (0.1\%)    &                       & 4 (0.3\%)  &  &
		\\ \hline
		NA (unpublished) &                       &              &                       &            & 1 (0.1\%) &
		\\ \hline
	\end{tabular}

==> figures/survey/table-data-sources-topics.tex <==

\footnotesize
% ./eqn.py -f coded-05.csv -t "data source" -c "topic"
	\newcolumntype{C}{>{\centering\arraybackslash}m{0.1\linewidth}}
	\begin{tabular}{l C C C C C C}
	                            & Research data provider & Partnership & Custom instrumentation & Not stated & MOOC & E-commerce
		\\ \hline
		Behavior profiling      & 18 (1.4\%)    & 83 (6.5\%)   & 34 (2.7\%)         & 15 (1.2\%) &      & 5 (0.4\%)
		\\ \hline
		Security and privacy    &               & 42 (3.3\%)   & 21 (1.6\%)         & 5 (0.4\%) &      &  
		\\ \hline
		Other                   & 1 (0.1\%)     & 4 (0.3\%)    &                    & 1 (0.1\%) &      &  
		\\ \hline
		Online sales and marketing & 94 (7.4\%) & 8 (0.6\%) & 1 (0.1\%)        &            &      & 260 (20.4\%)
		\\ \hline
		Metadiscussion          & 4 (0.3\%)     &              & 13 (1.0\%)         &            &      &  
		\\ \hline
		Health                  & 65 (5.1\%)    & 19 (1.5\%)   & 58 (4.5\%)         & 2 (0.2\%) &      &  
		\\ \hline
		Politics                & 43 (3.4\%)    & 4 (0.3\%)    & 7 (0.5\%)          & 4 (0.3\%) &      &  
		\\ \hline
		News consumption        & 3 (0.2\%)     & 8 (0.6\%)    & 8 (0.6\%)          &            &      &  
		\\ \hline
		Network analysis        & 1 (0.1\%)     & 10 (0.8\%)    & 31 (2.4\%)         &            &      &  
		\\ \hline
		HCI                     & 20 (1.6\%)    & 25 (2.0\%)   & 12 (0.9\%)         &            &      &  
		\\ \hline
		Recommender systems     & 1 (0.1\%)    & 15 (1.2\%)   &                    &            &      & 9 (0.7\%)
		\\ \hline
		Workplace               &               & 11 (0.9\%)   & 4 (0.3\%)          &            &      &  
		\\ \hline
		Financial               &               & 11 (0.9\%)   &                    &            &      &  
		\\ \hline
		Education               &               & 1 (0.1\%)    & 15 (1.2\%)         &            & 251 (19.7\%) &  
		\\ \hline
		Computer systems        &               & 10 (0.8\%)   & 19 (1.5\%)         &            &      &  
		\\ \hline
		\textbf{Total}     & \textbf{250 (19.6\%)} & \textbf{251 (19.7\%)} & \textbf{223 (17.5\%)} & \textbf{27 (2.1\%)} & \textbf{251 (19.7\%)} & \textbf{274 (21.5\%)}
		\\ \hline
	\end{tabular}

==> figures/survey/table-topics-stats.tex <==

\footnotesize
	\newcolumntype{C}{>{\centering\arraybackslash}m{0.17\linewidth}}
	% ./eqn.py -f coded-05.csv -t "relevant" -c "topic"
	\begin{tabular}{l C }
	    \textbf{Topic}                   & \textbf{Number of studies} \\ \hline
	    Online sales and marketing       & 363 (28.4\%) \\               \hline
	    Education                        & 267 (20.9\%) \\               \hline
	    Behavior profiling               & 155 (12.1\%) \\               \hline
	    Health                           & 144 (11.3\%) \\               \hline
	    Security and privacy             & 68 (5.3\%) \\                 \hline
	    Politics                         & 58 (4.5\%) \\                 \hline
	    HCI                              & 57 (4.5\%) \\                 \hline
	    Network analysis                 & 42 (3.3\%) \\                 \hline
	    Computer systems                 & 29 (2.3\%) \\                 \hline
	    Recommender systems              & 25 (2.0\%) \\                 \hline
	    News consumption                 & 19 (1.5\%) \\                 \hline
	    Metadiscussion of collection     & 17 (1.3\%) \\                 \hline
	    Workplace                        & 15 (1.2\%) \\                 \hline
	    Financial                        & 11 (0.9\%) \\                 \hline
	    Other                            & 6 (0.5\%) \\                  \hline
	\end{tabular}
